MURRE: Multi-Hop Table Retrieval with Removal for Open-Domain Text-to-SQL

The open-domain text-to-SQL task aims to retrieve question-relevant tables from massive databases and generate SQL. However, the performance of current methods is constrained by single-hop retrieval, and existing multi-hop retrieval of open-domain question answering is not directly applicable due to the tendency to retrieve tables similar to the retrieved ones but irrelevant to the question. Since the questions in text-to-SQL usually contain all required information, while previous multi-hop retrieval supplements the questions with retrieved documents. Therefore, we propose the multi-hop table retrieval with removal (MURRE), which removes previously retrieved information from the question to guide the retriever towards unretrieved relevant tables. Our experiments on two open-domain text-to-SQL datasets demonstrate an average improvement of 5.7% over the previous state-of-the-art results.

==> fig/pie.tex <==
\resizebox{0.75\linewidth}{!}{
    \begin{tikzpicture}[scale=0.6]
        \small
        \pie[
            pos={8,0},
            color={cblue!50, cpurple!80, white!20},
            text=legend
        ]{
            54.7/similar irrelevance,
            29.8/dissimilar relevance,
            15.5/other
        }
    \end{tikzpicture}
}

==> old_version/1.introduction_0913.tex <==
% text-to-SQL作为自然语言处理领域的重要任务，由于其降低了人们access数据库的门槛并且帮助人们高效查询数据，并且在金融、教育、商业等领域有着广泛应用。
Text-to-SQL, a significant task of natural language processing, reduces the difficulty of accessing databases and aids in efficient data querying, which has broad applications across many fields \cite{qin2022surveytexttosql}.
% 一个贴近现实场景的setting是open-domain text-to-SQL任务，which means系统需要面对海量数据将用户查询转换为SQL。
Unlike the previous text-to-SQL task that provides the question-relevant database tables\footnote{For brevity, we refer to database tables relevant to the question as \textbf{relevant tables} in this paper.}\cite{shi2024survey_text-to-sql-llm,hong2024nextgeneration-survey-text-to-sql}, a more realistic scenario is open-domain text-to-SQL, which should handle vast amounts of databases to convert user questions into SQL.
% 具体地，open-domain text-to-SQL需要根据问题从开放域数据库中检索到相关数据库及表格，即检索模块，再基于检索结果生成用户问题对应的SQL查询，即text-to-SQL模块。
Specifically, the open-domain text-to-SQL task involves two main steps: retrieving relevant tables and generating SQL based on the retrieved tables and the user question \cite{kothyari-etal-2023-crush4sql}.
% 为了简略，我们在本文简称和问题相关的表格schema为relevant schema，由于我们通常以表格schema代表表格被检索

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/intro.pdf}
    \caption{
        % 多跳表格检索中可能面临的挑战
        % Challenges in multi-hop table retrieval. 
        The two challenges of existing methods.
        % 相同的形状代表表格之间的相似度较高，绿色的表格代表相关表格，红色的表格代表不相关表格
        % 有相同形状的表格之间有较高的相似度
        The same shapes denote similar tables.
        The \introgreen{green} represents the relevant tables, and the \introred{red} represents the irrelevant.
        % 多跳检索（a）可能第一跳产生错误，导致错误级联；
        Multi-hop retrieval (a) gets irrelevant tables in the first hop, resulting in error cascades.
        % beam retrieval（b）可能即使第一跳检索到相关表格，在后续跳步检索到形似表格造成错误
        Multi-hop retrieval employing the beam search paradigm (b) retrieves tables in the second hop similar to the retrieved tables in the first hop but irrelevant to the question.
    }
    \vspace{-1.5em}
    \label{fig:intro}
\end{figure}


Considering the extensive knowledge embedded in LLM parameters, CRUSH~\cite{kothyari-etal-2023-crush4sql} bridges the semantic gap between natural language user questions and structured database tables by rewriting user questions into potentially relevant tables. 
However, CRUSH performs table retrieval in a single hop, limiting its performance because the retrieval of certain tables could depend on others, similar to multi-hop retrieval in the open-domain question answering (QA) task \cite{multi-hop-paragraph-retrieval,xiong2021Multi-Hop_Dense_Retrieval}. 
Nevertheless, directly adapting previous multi-hop retrieval methods to the open-domain text-to-SQL task presents two significant challenges, as illustrated in Figure~\ref{fig:intro}.


% 首先，检索器可能在多跳检索的前面检索到不相关的表，导致在后续检索中产生错误级联，就如图1中(a)
First, the retriever could retrieve irrelevant tables, leading to \textit{\textbf{error cascades}} in subsequent retrievals, as shown in Figure~\ref{fig:intro}(a). 
% 第二，检索器在多跳之间很容易检索和已经检索到的表格相似的表格，导致多跳检索失效，就像图1(b)右边部分一样
Second, the retriever could easily \textit{\textbf{retrieve tables that are similar to those retrieved in previous hops but irrelevant to the question}}, as illustrated in the right part of Figure~\ref{fig:intro}(b). 
% 开放域问答中，用户问题的信息可能不完整，需要检索得到的文档作为补充
This occurs because most multi-hop methods add the retrieved documents into the user question as the supplementary \cite{lee-etal-2022-generative_multi-hop,shao-etal-2023-enhancing_iterretgen}. 
% 而在开放域text-to-SQL中，由于表名或列名几乎不包含额外信息，因此用户问题中已经包含了检索所需的所有信息，使得在多跳检索时，为了避免检索到重复或相似的表，需要从问题中剔除掉已经检索到的表
Conversely, in open-domain text-to-SQL, the user question typically contains all necessary information for retrieval with no need for the supplementary. 
% 因此，将已经检索到的表格补充到用户问题中很容易导致后续检索到的表格和已检索到的表格很相似，导致检索性能较差
Consequently, adding retrieved tables to the question can cause retrieved tables similar to those already retrieved but irrelevant to the question, resulting in limited retrieval performance.
% 比如图1(b)右边部分中，如果将问题和employ表格拼接进行下一跳检索，那么和employ表格相似的表格staff会比相关表格bonus更容易被检索到
For instance, in the right part of Figure~\ref{fig:intro}(b), the irrelevant table "\textit{staff}" is retrieved because it is similar to the table "\textit{employee}" retrieved in the first hop.


% 因此，我们提出方法xxx，多跳表格检索，以增强开放域text-to-SQL的检索性能
To solve the above challenges, we propose a method called \textbf{MU}lti-hop table \textbf{R}etrieval with \textbf{R}ewrite and b\textbf{E}am search (\ourmethod) to enhance the retrieval performance for the open-domain text-to-SQL.
% 我们采用多跳表格检索方法，采用束搜索范式每跳维持多个并行检索，并改写用户问题移除已经检索到的表格信息，以进行下一跳检索
As illustrated in Figure~\ref{fig:intro}(c), our method retrieves tables through the multi-hop retrieval, adopting the beam search paradigm to maintain multiple retrievals per hop, inspired by \citet{zhang2023beam_retrieval}.
% 对于第一个挑战，我们引入了多跳表格检索，并且采用束搜索范式，在每一跳考虑多个可能的表格，减弱在前面跳步检索到不相关表格的影响
To address the error cascade, we employ the beam search paradigm to consider multiple possible tables at each hop, mitigating the impact of retrieving irrelevant tables in previous hops.
% 对于第二个挑战，我们提示LLM从用户问题中抽取出还未被检索到的表格信息以引导下一跳检索，缓解了检索到相似但不相关的表格的现象
For the second challenge, we prompt LLMs to remove the retrieved table information from the user question, forming a new question for the next hop, which reduces the retrieval of tables similar to the previously retrieved ones but irrelevant.


% （实验部分）
% 为了验证方法的有效性，我们在两个主流数据集spider和BIRD上进行实验
To validate the effectiveness of \ourmethod, we conduct experiments on two datasets, SpiderUnion and BirdUnion, which are open-domain versions of text-to-SQL datasets Spider~\cite{yu-etal-2018-spider} and Bird~\cite{li2023bird}.
% 相比较前人方法，我们的方法在两个数据集上得到了平均xx%的提升，证明了方法的有效性
\ourmethod achieves an average improvement of $5.7\%$ compared to the previous state-of-the-art (SOTA) results, demonstrating its effectiveness.
% 此外，分析实验证明，我们的方法可以提升开放域text-to-SQL的性能
Additionally, our case studies indicate that \ourmethod enhances the performance of the open-domain text-to-SQL by mitigating the two challenges mentioned above.


% （Contribution）
% 这篇文章的主要贡献如下：
Our contributions are as follows:
\begin{itemize}[nolistsep,leftmargin=*]
    % % 1.为了减轻多跳检索中错误级联的影响，我们提出多跳表格检索with束搜索范式，能够在每一跳考虑多个可能的表格，增加在每一跳检索到相关表格的概率
    % \item To mitigate the impact of error cascades in multi-hop retrieval, we propose utilizing the beam search paradigm, which reduces the impact of retrieving question-irrelevant tables.
    % % 2.为了缓解在多跳中反复检索到相似或重复的表格，我们提出从用户问题中移除已经检索到的表格信息得到下一跳的问题，w指导获取未被检索到的表格
    % \item To address the challenge of retrieving tables that are similar to previously retrieved ones but are irrelevant to the question, we propose removing the retrieved information from the user question, guiding the retriever to find new relevant tables.

    % 为了启发开放域text-to-SQL的研究，我们讨论了为什么多跳直接应用于text-to-SQL任务
    \item (Analysis)
    % 为了确保检索的表与用户问题相关，我们...
    \item (Methodology)
    % 3.为了验证我们方法的有效性，我们在spider和bird数据集上验证，取得了平均xx%的提升，证明了方法有效性
    \item To demonstrate the effectiveness of \ourmethod, we conduct experiments on the SpiderUnion and BirdUnion datasets, achieving an average improvement of $5.7\%$ compared with the previous SOTA results, proving its effectiveness.
\end{itemize}


==> old_version/1.introduction_0915.tex <==
% 第一段：开放域text-to-SQL的定义
% 第二段：介绍CRUSH，提出CRUSH没用多挑，给出用多跳的两个challenge
% 第三段：为了解决challenge，我们给出了我们的分析+方法
% 第四段：分析
% 第五段：方法
% 第六段：实验

% text-to-SQL作为自然语言处理领域的重要任务，由于其降低了人们access数据库的门槛并且帮助人们高效查询数据，并且在金融、教育、商业等领域有着广泛应用。
Text-to-SQL, which simplifies database access and facilitates efficient data querying, is an important task in natural language processing \cite{qin2022surveytexttosql}.
% 一个贴近现实场景的setting是open-domain text-to-SQL任务，which means系统需要面对海量数据将用户查询转换为SQL。
Unlike the previous text-to-SQL task that provides the question-relevant database tables\footnote{For brevity, we refer to database tables relevant to the question as \textbf{relevant tables} in this paper.} \cite{yu-etal-2018-spider,shi2024survey_text-to-sql-llm}, a more realistic scenario involves open-domain text-to-SQL, where user questions are transformed into SQL across vast databases.
% 具体地，open-domain text-to-SQL需要根据问题从开放域数据库中检索到相关数据库及表格，即检索模块，再基于检索结果生成用户问题对应的SQL查询，即text-to-SQL模块。
Therefore, open-domain text-to-SQL necessitates two main steps: retrieving relevant tables and generating SQL based on the retrieved tables and user question \cite{kothyari-etal-2023-crush4sql}.
% 为了简略，我们在本文简称和问题相关的表格schema为relevant schema，由于我们通常以表格schema代表表格被检索


\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/intro.pdf}
    \caption{
        % 多跳表格检索中可能面临的挑战
        % Challenges in multi-hop table retrieval. 
        The comparison between multi-hop retrieval with supplementary and exclusive rewriting.
        % 相同的形状代表表格之间的相似度较高，绿色的表格代表相关表格，红色的表格代表不相关表格
        % 有相同形状的表格之间有较高的相似度
        The same shapes denote similar tables.
        % The \introgreen{green} represents the relevant tables, and the \introred{red} represents the irrelevant.
        % 多跳检索with补充改写（a）即使第一跳检索到相关表格，在后续跳步检索到形似表格造成错误；
        % Multi-hop retrieval with supplementing the question retrieves tables similar to the previously retrieved tables but irrelevant to the question.
        Multi-hop retrieval that supplements the question retrieves tables similar to those already retrieved, even if they are irrelevant to the question.
        % 多跳检索with移除改写（b）能够在第二跳检索到其他相关表格
        In contrast, multi-hop retrieval with exclusive rewriting can successfully retrieve other relevant tables in the second hop.
    }
    \vspace{-1.5em}
    \label{fig:intro}
\end{figure}


To bridge the semantic gap between natural language user questions and structured database tables, CRUSH~\cite{kothyari-etal-2023-crush4sql} rewrites the user question into potentially relevant tables for retrieval. 
However, CRUSH retrieves tables in a single hop, limiting its performance because the retrieval of certain tables could depend on others, similar to multi-hop retrieval in other tasks \cite{multi-hop-paragraph-retrieval,xiong2021Multi-Hop_Dense_Retrieval}. 
Nevertheless, directly adapting previous multi-hop retrieval methods could easily \textit{\textbf{retrieve tables that are similar to those retrieved in previous hops but irrelevant to the question}} since previous multi-hop retrieval usually supplements the retrieved documents into the user question \cite{shao-etal-2023-enhancing_iterretgen,rag_survey_2024,jeong2024adaptiverag}, as illustrated in Figure~\ref{fig:intro}.
% 首先，检索器可能在多跳检索的前面检索到不相关的表，导致在后续检索中产生错误级联，影响,就如图1中(a)
% First, the retriever could retrieve irrelevant tables, leading to \textit{\textbf{error cascades}}, which affect subsequent retrievals, as shown in Figure~\ref{fig:intro}(a). 
% 第二，检索器在多跳之间很容易检索和已经检索到的表格相似的表格，导致多跳检索失效，就像图1(b)右边部分一样
% The retriever could easily \textit{\textbf{retrieve tables that are similar to those retrieved in previous hops but irrelevant to the question}} since previous multi-hop retrieval usually supplements the retrieved documents into the user question \cite{shao-etal-2023-enhancing_iterretgen,rag_survey_2024,jeong2024adaptiverag}.
% 开放域问答中，用户问题的信息可能不完整，需要检索得到的文档作为补充
% This occurs because most multi-hop methods add the retrieved documents into the user question as the supplementary \cite{lee-etal-2022-generative_multi-hop,shao-etal-2023-enhancing_iterretgen}. 
% 而在开放域text-to-SQL中，由于表名或列名几乎不包含额外信息，因此用户问题中已经包含了检索所需的所有信息，使得在多跳检索时，为了避免检索到重复或相似的表，需要从问题中剔除掉已经检索到的表
% Conversely, in open-domain text-to-SQL, the user question typically contains all necessary information for retrieval with no need for the supplementary. 
% 因此，将已经检索到的表格补充到用户问题中很容易导致后续检索到的表格和已检索到的表格很相似，导致检索性能较差
% Consequently, adding retrieved tables to the question can cause retrieved tables similar to those already retrieved but irrelevant to the question, resulting in limited retrieval performance.
% 前人工作经常将检索到的文档补充进用户问题，以继续检索相关文档。
% 然而，开放域text-to-SQL的问题中通常包含全部需要的信息，再补充检索到的表格会导致倾向于检索和已经检索到的表格相似的表格，而非其他相关的表格
However, the user question of the open-domain text-to-SQL typically contains all necessary information in open-domain text-to-SQL.
% , causing retrieved tables similar to the previously retrieved tables but irrelevant if the retrieved information is added to the question. 
% 比如图1(b)右边部分中，如果将问题和employ表格拼接进行下一跳检索，那么和employ表格相似的表格staff会比相关表格bonus更容易被检索到
For instance, in the left part of Figure~\ref{fig:intro}, the irrelevant table "\textit{staff}" is retrieved because it is similar to the table "\textit{employee}" retrieved in the first hop.

% 为了解决上述问题，我们关注于分析适用于开放域text-to-SQL的多跳方法，从以下两个方面
To solve the above problem, we focus on exploring the multi-hop table retrieval method applicable to open-domain text-to-SQL, from the following two aspects.
% （1）我们分析了为什么其他任务的多跳检索方法无法直接应用于开放域text-to-SQL任务
(\emph{i})~We analyze why the multi-hop retrieval methods of other tasks cannot be directly applied to open-domain text-to-SQL.
% （2）我们提出基于改写的多跳检索，来确保每一跳检索的结果都和用户问题而非之前跳步检索的结果相关
(\emph{ii})~We propose a multi-hop table retrieval method based on rewriting for open-domain text-to-SQL, to ensure that the retrieved tables of each hop are relevant to the user question rather than the previously retrieved tables.

% 我们首先分析了为什么其他任务的多跳检索不能直接用于开放域text-to-SQL
We first discuss that multi-hop retrieval of other tasks cannot be directly used for open-domain text-to-SQL.
% 我们首先总结了其他任务中的多跳检索方法，通常在每一跳将检索到的信息补充进问题中
% We summarize the multi-hop retrieval method in other tasks, where the questions in each hop are usually supplemented with information retrieved in previous hops.
% 而考虑到开放域text-to-SQL和其他任务的不同，我们的问题无需检索到的表格信息作为补充
% Considering the difference between open-domain text-to-SQL and other tasks, our questions do not need the retrieved table information as a supplement.
% 实验结果表明，直接沿用前人工作将检索到的表格和问题拼接作为下一跳的问题会导致多跳检索性能很差，甚至不如单跳检索的性能，证明了前人工作的不适用
% The experimental results also show that directly following previous works leads to poor performance, proving the inapplicability of multi-hop retrieval in other tasks.
% 1. 我们首先分析了前人的多跳检索主要是将检索结果补充到用户问题中；
We analyze that existing multi-hop retrieval methods are mainly to supplement the retrieval results to the user question.
% 2. 然而，我们提出开放域text-to-SQL需要剔除而非补充信息，因为用户问题中已经包含了所有需要的信息
However, open-domain text-to-SQL needs to exclude retrieved information rather than supplement it because all the necessary information is involved in the user question.
% 3. 我们给出了分析实验，来证明我们的观点
We conduct analysis experiments to prove our point of view.


% 因此，我们提出方法xxx，多跳表格检索，以增强开放域text-to-SQL的检索性能
Based on the above discussion, we propose a method called \textbf{MU}lti-hop table \textbf{R}etrieval with \textbf{RE}write (\ourmethod), to enhance the performance of open-domain text-to-SQL through multi-hop retrieval.
% 我们采用多跳表格检索方法，采用束搜索范式每跳维持多个并行检索，并改写用户问题移除已经检索到的表格信息，以进行下一跳检索
% 我们的方法在多跳检索表时，通过改写和beam来确保检索的表与问题相关
As presented in the right part of Figure~\ref{fig:intro}, \ourmethod searches relevant tables employing multi-hop retrieval, by rewriting questions excluding the retrieved table information from the question to ensure retrieved tables relevant to the user question.
% 对于第一个挑战，我们引入了多跳表格检索，并且采用束搜索范式，在每一跳考虑多个可能的表格，减弱在前面跳步检索到不相关表格的影响
% To address the error cascades, we employ the beam search paradigm to consider multiple possible tables at each hop, mitigating the impact of retrieving irrelevant tables in previous hops.
% 对于第二个挑战，我们提示LLM从用户问题中抽取出还未被检索到的表格信息以引导下一跳检索，缓解了检索到相似但不相关的表格的现象
% Specifically, we prompt LLMs to remove the retrieved table information from the user question, forming a new question for the next hop, which reduces the retrieval of tables similar to the previously retrieved ones but irrelevant.


% （实验部分）
% 为了验证方法的有效性，我们在两个主流数据集spider和BIRD上进行实验
To validate the effectiveness of \ourmethod, we conduct experiments on two datasets, SpiderUnion and BirdUnion, which are open-domain versions of text-to-SQL datasets Spider~\cite{yu-etal-2018-spider} and Bird~\cite{li2023bird}.
% 相比较前人方法，我们的方法在两个数据集上得到了平均xx%的提升，证明了方法的有效性
\ourmethod achieves an average improvement of $5.7\%$ compared to the previous state-of-the-art (SOTA) results, demonstrating its effectiveness.
% 此外，分析实验证明，我们的方法可以提升开放域text-to-SQL的性能
% Additionally, our analysis experiments indicate that \ourmethod can mitigate the challenge mentioned above.
% 此外，我们统计了检索结果的平均排名，证明了我们的方法能有效地检索出和已检索结果不相关的表，证明了我们的方法确实可以移除已检索的信息
Additionally, we count the average rank of the retrieval results, proving that \ourmethod can effectively retrieve tables that are not similar to the retrieved results, and prove that our method can indeed exclude the retrieved information.


% （Contribution）
% 这篇文章的主要贡献如下：
Our contributions are as follows:
\begin{itemize}[nolistsep,leftmargin=*]
    % 为了启发开放域text-to-SQL的研究，我们讨论了为什么多跳不能直接应用于text-to-SQL任务
    \item To inspire the research of open-domain text-to-SQL, we discuss why multi-hop retrieval in other tasks can not be directly applied to text-to-SQL.
    % 为了确保检索的表与用户问题相关，我们在每一跳将检索到的信息从问题中移除，并采用束搜索范式
    \item To ensure that the retrieved tables are relevant to the user question, we rewrite the question by excluding the retrieved information at each hop.
    % 3.为了验证我们方法的有效性，我们在spider和bird数据集上验证，取得了平均xx%的提升，证明了方法有效性
    \item To demonstrate the effectiveness of \ourmethod, we conduct experiments on the SpiderUnion and BirdUnion datasets, achieving an average improvement of $5.7\%$ compared with the previous SOTA results, proving its effectiveness.
\end{itemize}


==> old_version/2.methodology_0904.tex <==
\subsection{Task Definition}
    % 任务定义，方法简要描述
    Our work mainly focuses on the open-domain text-to-SQL task, which can be formally defined as:
    % 给定用户问题和大量表格，我们方法目标是检索到用户问题相关的表格
    Given a user question $q$, database tables $T=\{t_i\}$ and a number of retrieved tables $N$, suppose the tables relevant to $q$ are $T^q = \{t^q_i\}$, \ourmethod aims to retrieve $N$ tables $T^{q}_N$, where $T^q \subseteq T^{q}_N$.

\subsection{Overview}
    The overview of \ourmethod is illustrated in Figure~\ref{fig:method}.
    % 我们的方法由H个跳步组成，每一跳包括B个束搜索，同时又分为两个阶段：检索和改写
    \ourmethod comprises multiple hops, with each hop consisting of several beams.
    Each hop can be divided into two phases: \textbf{Retrieve} (\S\ref{subsec:retrieve}) and \textbf{Rewrite} (\S\ref{subsec:rewrite}).
    % 在每跳，我们首先通过计算和用户问题相关的概率检索相关表格
    In each hop, we first \textbf{retrieve} the relevant tables by calculating their probability that is relevant to the question.
    % 然后，我们基于用户问题和检索结果，通过改写删除用户问题中被检索表的信息，来得到新一轮的用户问题
    Next, using the original user question and the retrieved tables in each beam, we \textbf{rewrite} the user question to exclude the information of the retrieved tables, generating the user question used for the subsequent hop.
    % 我们重复以上检索过程直到达到最大跳步数，或满足早停条件, which is discussed in rewrite subsection
    \ourmethod repeats the Retrieve and Rewrite phases until reaching the maximum hop limit $H$ or meeting the early stop condition (see \S\ref{subsec:rewrite}).
    % 在检索完成后，我们根据检索过程中的相似度对每个表格打分重新排序
    After the multi-hop retrieval, we \textbf{score} (\S\ref{subsec:rank}) each table based on its probability that is relevant to the user question and select the top-$N$ tables as the input for generating the SQL.
    % 在附录中，我们还讨论了如果数据库中没有与用户问题相关的表格的情况
    In Appendix~\ref{appendix:no relevant tables}, we explore how to handle the situation when no table in the database is relevant to the user question.
    

\subsection{Retrieve}
\label{subsec:retrieve}
    The Retrieve phase aims to identify $B$ tables corresponding to the user question $q^{h,b}$, where $B$ is the beam size and $q^{h,b}$ denotes the user question at hop $h$ and beam $b$. 
    We embed the user question and each table into vectors and then compute their relevance probability to the user question. 
    Let \texttt{Emb}($x$) represent the embedding vector of $x$, the probability is expressed as Equation~\ref{equ:p_hat}. 
    \begin{equation}
        \hat{P}(t_i | q^{h,b}) = \texttt{Norm}(\frac{\texttt{Emb}(t_i) \cdot \texttt{Emb}(q^{h,b})}{|\texttt{Emb}(t_i)||\texttt{Emb}(q^{h,b})|})
        \label{equ:p_hat}
    \end{equation}
    % 即问题和表格向量间的余弦相似度，具体的表格表示形式和归一化方式分别见Appendix~\ref和Appendix~\ref
    We use the cosine similarity between the question and table vectors to calculate the probability, adopting $\texttt{Norm}$ to ensure the conditional probabilities sum to one. 
    Detailed representations of the table and the normalization method are provided in Appendix~\ref{appendix:prompts for rewrite} and Appendix~\ref{appendix:normalization method}, respectively. 
    % 我们选取相似度最高的B个结果，作为q^{h,b}相应的检索结果
    We select the $B$ tables with the highest probabilities as the retrieval results for the current hop question $q^{h,b}$.

    % 由于上一轮检索中，每个beam都会对应一个q^{h,b}，因此总共会有b \times b个结果
    In the previous hop of retrieval, there are $B$ beams and each beam corresponds to $B$ retrieved tables obtained at the current hop, resulting in a total of $B \times B$ retrieval results.
    % 我们从中选取B个结果，用于后续的改写，具体的选取方法见\S\ref
    Following the beam search paradigm, we then choose $B$ results from these for the subsequent rewriting phase, with the selection method detailed in \S\ref{subsec:rank}.

\subsection{Rewrite}
\label{subsec:rewrite}
    % 改写阶段是为了从用户问题中剔除出当前轮检索到的表格的信息，将未检索到的信息表示成表格的形式，作为下一跳的用户问题，来引导模型去检索问题相关但还没有被检索到的表
    % path是从第一跳开始检索到第h跳在第b束的路径上的所有被检索到的表
    The Rewrite phase is designed to mitigate the retrieval of tables that are similar to previously retrieved ones yet irrelevant to the user question.
    To achieve the above goal, this phase employs LLMs to rewrite the user question, by removing the information of retrieved tables in $\texttt{Path}^{h,b}$ (which includes all retrieved tables from hop $1$ to hop $h$ on the path of beam $b$) from the user question $q$, and express the unretrieved information in the form of a table following the previous work \cite{kothyari-etal-2023-crush4sql}, where the rewritten question is used to guide the retriever for the next hop.
    % in retrieving tables relevant to $q$ but not yet retrieved. 

    % 由于每个用户问题需要查询的表格数量不同，为避免额外的跳步引入错误，我们希望系统能够自动判断检索到的表格是否足够回答问题，即早停机制
    Considering that different user questions require varying numbers of tables, to prevent additional hops from introducing errors, we instruct LLMs to assess whether the retrieved tables in $\texttt{Path}^{h,b}$ are sufficient to answer $q$, i.e., early stop. 
    % 我们设置的早停条件如下：提示LLM生成一个特殊的mark来表示目前已经检索完全，并且与其对应相同原始用户问题的其它beam_size-1个检索也在这一跳停止
    In detail, we prompt the LLM to generate a special mark (e.g., "None" in Figure~\ref{fig:method}) during rewriting to indicate that the retrieved tables are sufficient to answer the user question $q$, ceasing further retrieval as soon as this early stop mark is produced.
    The prompts used for rewriting are detailed in Appendix~\ref{appendix:prompts for rewrite}.

    % \begin{algorithm*}[t]
    %     % \small
    %     \begin{algorithmic}[1]
    %         \item[] {\bfseries Input:}
    %             The similarity corresponding to each table $t$ in each hop $h$: $all\_paths=[[(table_{11}, score_{11}), \ldots, (table_{1H}, score_{1H})]$$, \ldots, 
    %             [(table_{P1}, score_{P1}), \ldots, 
    %             (table_{PH}, $$score_{PH})]]$, 
    %             the number of max hops $H$, 
    %             the number of all paths $P$.
    %         \item[] {\bfseries Output:}
    %             The scores of each table $t$
    %         \STATE  Initialization : $table\_score \gets \left\{\right\}$
    %         \FOR{$each\_path$ in $all\_paths$}
    %             \STATE $score \gets 1$
    %             % 将分数初始化，便于后续累乘
    %             \COMMENT{Initialize the score}
    %             \FOR{$example$ in $each\_path$}
    %                 \STATE $score = \adam{score \times example\left[1\right]}$
    %                 \COMMENT{Calculate the score of the path}
    %                 % 计算列表中表格分数的累乘
    %             \ENDFOR
    %             \FOR{$example$ in $each\_path$}
    %                 \STATE {\begin{tabular}[t]{@{}l@{}}$table\_score\left[example\left[0\right]\right] \gets$$\adam{max(score,$ $table\_score\left[example\left[0\right]\right])}$\end{tabular}} \\
    %                 \COMMENT{Update the table score with the max path score}
    %                 % \COMMENT{select batch and return the corresponding gradient}
    %             \ENDFOR
    %         \ENDFOR
    %         \RETURN $table\_score$
    %     \end{algorithmic}
    %     \caption{The \adamtext{table scoring} algorithm in \ourmethod}
    %     \label{alg:algorithm}
    % \end{algorithm*}

\subsection{Score}
\label{subsec:rank}
    The aforementioned multi-hop retrieval process maintains $B$ paths at each hop, containing tables that could exceed or fall short of the required number of tables $N$. 
    % Rank阶段的目的是根据Retrieve阶段的检索结果来进行打分，从而保留指定数量的检索结果，其包含两个部分：
    Therefore, this phase aims to score all the tables based on their probabilities to retain the most relevant tables used for generating SQL, which consists of two parts: 
    % 1. 根据检索路径得到该检索路径的分数：Rank_Path((q^{1,b}, t^{q^{1, b}}_{i}), ..., (q^{h,b}, t^{q^{h, b}}_{i})\})
    (\emph{i}) scoring the retrieval path $\texttt{Score\_Path}(\texttt{Path}^{h,b})$;
    % 2. 根据所有某个表相关的路径的分数来得到表t的分数：Rank_Table(t)
    (\emph{ii}) scoring the retrieved table $\texttt{Score\_Table}(t_i)$.
    
    \paragraph{Retrieval Path Score}
        % 首先，我们讨论如何计算一个检索路径的分数，这里的检索路径上的每个节点对应每个hop的某个beam上的检索结果
        First, we address the calculation of the retrieval path score, where each node on the path corresponds to the retrieved table on a beam of one hop. 
        % 根据\S\ref中的讨论，每个检索路径的分数可以被看作为，路径上最后一个表格被检索到的概率，在它对应的用户问题的条件下
        As discussed in \S\ref{subsec:retrieve}, the score of each retrieval path represents the probability that the last table in the path is retrieved, given its corresponding question at the last hop. 
        % 经过推导，检索路径的分数即为检索路径上所有表格依次被检索到的概率乘积，具体的推导过程见附录C
        Following the derivation in Appendix~\ref{appendix:score of the retrieval path}, the score of a retrieval path is computed as the product of all the probabilities $\hat{P}$ in the path.

        
    \paragraph{Table Score}
        % 在计算路径分数的基础上，我们讨论如何计算给定表t的分数
        Building on the retrieval path score, we describe the calculation to score a retrieved table $t_i$. 
        % 因为每个表格可能在多跳、多束中被多次检索，所以我们提出一个表格打分算法，合理集成每个表格对应的检索路径的分数
        Since each table has multiple scores across various hops and beam retrievals, we propose a table scoring algorithm to effectively integrate these scores.
        Detailed information is provided in Appendix~\ref{appendix:table scoring algorithm}. 
        % 具体来说，由于问题相关的表格可能有多个，因此我们希望选取多个可能的表格，which互相关联，而一条路径的分数越高，证明路径中每个表格和问题的相关性越高，因此我们希望按照推理路径的分数由高到低排序作为结果
        Considering the potential interrelation of question-relevant tables, we aim to ensure that all retrieved tables collectively are the most relevant to the question.
        Thus, the higher the retrieval path score, the higher the score of the tables in the path. 
        % 相应的，令Path_t表示所有包含表格t的检索路径，则有：Rank_Table(t) = \mathop{\max}_{p \in Path_t} Rank_Path(p)
        Specifically, let $\texttt{Path}_{t_i}$ denote all retrieval paths containing table $t_i$, we calculate the table score as: $\texttt{Score\_Table}(t_i) = \mathop{\max}_{t \in Path_{t_i}} \texttt{Score\_Path}(t)$. 
        % 最终，我们选取分数最高的N个结果T^Q_N作为我们的检索结果
        Finally, we select $T^Q_N = \{t_1, ..., t_N\}$ with the highest $\texttt{Score\_Table}(t_i)$ as our retrieval results. 
        % 在附录中，我们展示了如何提升我们的表格打分算法，用于处理在用户问题或表格中存在的模糊实体或同义词的情况
        Appendix~\ref{appendix:synonyms} elaborates on enhancing the table scoring algorithm to address ambiguous entities or synonyms in user questions or tables.

==> old_version/3.experiments_0910.tex <==
    
    \subsection{Experiment Setup} 
    \begin{table}[t]
        \centering
        \small
        \begin{tabular}{l|ccccc}
            \toprule
            \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{5}{|c}{\textbf{\#table}}\\
             & \bm{$1$} & \bm{$2$} & \bm{$3$} & \bm{$4$} & \textbf{All} \\
            \midrule
            SpiderUnion & $395$ & $214$ & $43$ & $6$ & $658$\\
            BirdUnion & $364$ & $943$ & $207$ & $20$ & $1534$\\ 
            \bottomrule
        \end{tabular}
        \caption{
            Statistics on the number of the relevant table for each question in the SpiderUnion and BirdUnion.
            \textbf{\#table} denotes the number of the relevant table.
            \textbf{All} refers to the total number of questions in the dataset.
        }
        \label{tab:dataset}
    \end{table}

        \begin{table*}[t]
        \centering
        \small
        \begin{tabular}{lll|cccc|cccc}
            \toprule
            \textbf{Dataset} & \textbf{Model} & \textbf{Method} & \bm{$k=3$} &  \bm{$k=5$} &  \bm{$k=10$} &  \bm{$k=20$} & \bm{$r@3$} & \bm{$r@5$} & \bm{$r@10$} & \bm{$r@20$}\\
            \midrule
            \multirow{6}{*}{SpiderUnion} & \multirow{3}*{SGPT-125M} & Single-hop &  $54.3$ & $66.0$ & $75.4$ & $82.2$ & $63.0$ & $73.1$ & $80.7$ & $86.3$ \\
            ~ & ~ & CRUSH$^\dag$ & $60.2$ & $71.3$ & $80.7$ & \bm{$86.8$} &  $68.9$ & $76.3$ & \bm{$83.4$} & \bm{$88.9$}\\
            ~ & ~ & \ourmethod &  \bm{$65.0$} & \bm{$74.2$} & \bm{$81.0$} & $85.3$ & \bm{$70.2$} & \bm{$77.5$} & $82.3$ & $86.9$\\
            \cmidrule{2-11}
            ~ &  \multirow{3}{*}{SGPT-5.8B} & Single-hop &  $76.3$ & $86.8$ & $94.1$ & \bm{$97.6$} & $84.0$ & $91.5$ & $96.2$ & \bm{$98.7$}\\
            ~ & ~ & CRUSH$^\dag$ & $68.2$ &  $80.1$ & $88.4$ & $92.2$ & $75.5$ & $85.1$ & $91.2$ & $94.5$ \\
            ~ & ~ & \ourmethod & \bm{$86.0$} & \bm{$93.5$} & \bm{$96.7$} & $97.3$ & \bm{$89.3$} & \bm{$94.3$} & \bm{$96.8$} & $97.5$\\
            \midrule
            \multirow{6}{*}{BirdUnion} & \multirow{3}*{SGPT-125M} & Single-hop & $39.0$ & $50.3$ & $62.1$ & $70.9$ & $54.0$ & $63.2$ & $73.3$ & $80.9$ \\
            ~ & ~ & CRUSH$^\dag$ & $42.1$ & $56.1$ & $70.2$ & $77.7$ & $60.2$ & $70.0$ & $79.5$ & \bm{$86.1$} \\
            ~ & ~ & \ourmethod & \bm{$51.4$} & \bm{$62.7$} & \bm{$72.9$} & \bm{$78.3$} & \bm{$64.8$} & \bm{$72.7$} & \bm{$79.6$} & $84.2$\\
            \cmidrule{2-11}
            ~ &  \multirow{3}{*}{SGPT-5.8B} & Single-hop & $55.3$ & $67.3$ & $79.4$ & $86.4$ & $72.9$ & $80.8$ & $88.6$ & $92.8$ \\
            ~ & ~ & CRUSH$^\dag$ & $52.2$ &  $63.5$ & $78.4$ & $88.1$ & $70.0$ & $77.9$ & $87.5$ & $93.0$ \\
            ~ & ~ & \ourmethod & \bm{$69.1$} & \bm{$80.1$} & \bm{$88.7$} & \bm{$92.7$} & \bm{$81.0$} & \bm{$87.6$} & \bm{$92.6$} & \bm{$95.4$}\\
            \bottomrule
        \end{tabular}
        \caption{
            The main results on complete recall and recall of \ourmethod, compared with Single-hop and CRUSH on SpiderUnion and BirdUnion, using SGPT-125M and SGPT-5.8B as the embedding models. 
            $k$ refers to the complete recall, and $r$ refers to the recall.
            $^\dag$ denotes our run since the performance difference led by the API change.
            The best results of different datasets and models are annotated in \textbf{bold}.
        }
        \label{tab:main result}
    \end{table*}

    % \begin{table}[ht]
    %     \centering
    %     \small
    %     \begin{tabular}{lll|cccc}
    %         \toprule
    %         \textbf{Dataset} & \textbf{Model} & \textbf{Method} & \bm{$3$} &  \bm{$5$} &  \bm{$10$} &  \bm{$20$}\\
    %         \midrule
    %         \multirow{4}{*}{BirdUnion+} & \multirow{2}*{SGPT-125M} & Baseline & $11.0$ & $12.5$ & $15.4$ & $16.2$\\
    %         ~ & ~ & \ourmethod & \bm{$15.7$} & \bm{$17.1$} & \bm{$19.0$} & \bm{$18.1$}\\
    %         \cmidrule{2-7}
    %         ~ &  \multirow{2}{*}{SGPT-5.8B} & Baseline & $15.7$ & $17.7$ & $19.0$ & $19.5$\\
    %         ~ & ~ & \ourmethod & \bm{$20.3$} & \bm{$21.5$} & \bm{$22.2$} & \bm{$21.9$}\\
    %         \midrule
    %         \multirow{4}{*}{SpiderUnion} & \multirow{2}*{SGPT-125M} & Baseline &  $43.2$ & $48.2$ & $50.8$ & $52.7$\\
    %         ~ & ~ & \ourmethod &  \bm{$50.8$} & \bm{$52.9$} & \bm{$54.6$} & \bm{$56.5$}\\
    %         \cmidrule{2-7}
    %         ~ &  \multirow{2}{*}{SGPT-5.8B} & Baseline &  $55.3$ & $57.4$ & $60.3$ & $57.8$ \\
    %         ~ & ~ & \ourmethod & \bm{$59.9$} & \bm{$62.5$} & \bm{$63.5$} & \bm{$62.3$}\\
    %         \bottomrule
    %     \end{tabular}
    %     \caption{
    %         EX for predicted SQL with the input consisting of the user question and different numbers of retrieved tables.
    %     }
    %     \label{tab:text-to-sql}
    % \end{table}

    \paragraph{Dataset}
        To evaluate the effectiveness of \ourmethod, we validate it on two open-domain text-to-SQL datasets: SpiderUnion~\cite{kothyari-etal-2023-crush4sql} and BirdUnion, which mix all tables of Spider~\cite{yu-etal-2018-spider} and Bird~\cite{li2023bird}.
        Table~\ref{tab:dataset} shows the number of questions requiring different numbers of tables.
        Detailed descriptions of Spider and Bird are provided in Appendix~\ref{appendix:dataset details}.

    \paragraph{Metric}
        We employ recall and complete recall as evaluation metrics for retrieval, and Execution Accuracy (EX) \cite{yu-etal-2018-spider} for text-to-SQL. 
        Recall (\bm{$r@$}) measures the proportion of relevant tables retrieved from all relevant tables, following previous work \cite{kothyari-etal-2023-crush4sql}.
        Unlike other open-domain tasks (e.g., open-domain QA), it is crucial to retrieve all relevant tables to generate correct SQL for the open-domain text-to-SQL. 
        Hence, we introduce complete recall (\bm{$k=$}), which is the proportion of examples retrieving all relevant tables.
        For text-to-SQL, we use execution match (EX), following previous work~\cite{gao2023texttosqldail}, to evaluate the correctness of the execution results of predicted SQL compared to gold SQL.
    
    \paragraph{Model}
        We utilize SGPT~\cite{muennighoff2022sgpt} to embed tables and user questions without additional fine-tuning, following the previous work~\cite{kothyari-etal-2023-crush4sql}.
        For the Rewrite phase and SQL generation, we use \texttt{gpt-3.5-turbo}\footnote{\href{https://platform.openai.com/docs/models/gpt-3-5}{Document} for \texttt{gpt-3.5-turbo}} to predict.  
        % And for text-to-SQL, we employ \texttt{gpt-3.5-turbo} to generate SQL.
        The detailed descriptions of SGPT and \texttt{gpt-3.5-turbo} are provided in Appendix~\ref{appendix:model details}.

    \paragraph{Comparing System}
        In our experiments, we compare \ourmethod with the following methods: 
        (\emph{i}) Single-hop, which retrieves with the user question in a single hop;
        (\emph{ii}) CRUSH~\cite{kothyari-etal-2023-crush4sql}, which retrieves in a single hop with hallucinating the user question into the table format.

    \paragraph{Implement Details}
        We set the beam size to $5$, as it provides the best performance with the smallest size (see \S\ref{subsubsec:beam size}).
        % 简写为max hop
        The maximum hop (abbreviated as max hop) is set to $3$ because over $98\%$ of questions in the SpiderUnion and BirdUnion datasets require $\leq 3$ tables (see Table~\ref{tab:dataset}).
        % 因为BirdUnion中的表格规模比SpiderUnion的大
        We rewrite user questions using the $9$-shot prompt and $8$-shot prompt on the SpiderUnion and BirdUnion respectively, since the table scales of BirdUnion are larger than that of SpiderUnion.
        
    % \begin{table}[ht]
    %     \centering
    %     \small
    %     \begin{tabular}{ll|cccc}
    %         \toprule
    %         \textbf{Model} & \textbf{Method} & \bm{$3$} & \bm{$5$} & \bm{$10$} & \bm{$20$} \\
    %         \midrule
    %         \multirow{2}*{SGPT-125M} & baseline & $43.2$ & $48.2$ & $50.8$ & $52.7$ \\
    %         ~ & \ourmethod &  \bm{$50.8$} & \bm{$52.9$} & \bm{$54.6$} & \bm{$56.5$} \\
    %         \cmidrule{2-6}
    %         \multirow{2}{*}{SGPT-5.8B} & baseline &  $55.3$ & $57.4$ & $60.3$ & $57.8$ \\
    %         ~ & \ourmethod & \bm{$59.9$} & \bm{$62.5$} & \bm{$63.5$} & \bm{$62.3$} \\
    %         \bottomrule
    %     \end{tabular}
    %     \caption{
    %         EX for predicted SQL with the input, which includes the user question and different numbers of retrieved top tables on the SpiderUnion.
    %         The best results with different models are annotated in \textbf{bold}.
    %     }
    %     \label{tab:text-to-sql}
    % \end{table}

    % \begin{table*}[htbp]
    %     \centering
    %     \small
    %     \begin{tabular}{lll|cccc}
    %         \toprule
    %         \textbf{Dataset} & \textbf{Model} & \textbf{Method} & \bm{$r@3$} &  \bm{$r@5$} & \bm{$r@10$} & \bm{$r@20$}\\
    %         \midrule
    %         \multirow{6}{*}{SpiderUnion} & \multirow{2}*{SGPT-125M} & Single-hop &  $43.9$ & $50.0$ & $53.2$ & $54.1$ \\
    %         ~ & ~ & CRUSH & $47.3$ & $50.9$ & \bm{$55.9$} & \bm{$59.6$}\\
    %         ~ & ~ & \ourmethod & \bm{$50.3$} & \bm{$54.1$} & $54.7$ & $57.4$\\
    %         \cmidrule{2-7}
    %         ~ &  \multirow{3}{*}{SGPT-5.8B} & Single-hop & $54.9$ & $60.6$ & $61.6$ & $63.7$\\
    %         ~ & ~ & CRUSH & $49.8$ & $56.4$ & $60.3$ & $60.8$\\
    %         ~ & ~ & \ourmethod & \bm{$62.5$} & \bm{$64.4$} & \bm{$64.4$} & \bm{$66.7$}\\
    %         \midrule
    %         \multirow{6}{*}{BirdUnion} & \multirow{2}*{SGPT-125M} & Single-hop & $11.2$ & $13.4$ & $17.1$ & $18.5$\\
    %         ~ & ~ & CRUSH & $14.5$ & \bm{$17.1$} & $19.0$ & \bm{$20.5$}\\
    %         ~ & ~ & \ourmethod & \bm{$16.0$} & $16.8$ & \bm{$19.4$} & $20.0$\\ 
    %         \cmidrule{2-7}
    %         ~ &  \multirow{3}{*}{SGPT-5.8B} & Single-hop & $16.9$ & $17.3$ & $18.3$ & $20.4$\\
    %         ~ & ~ & CRUSH & $16.8$ & $18.0$ & $19.7$ & $21.1$\\
    %         ~ & ~ & \ourmethod & \bm{$20.9$} & \bm{$21.8$} & \bm{$22.0$} & \bm{$22.4$}\\
    %         \bottomrule
    %     \end{tabular}
    %     \caption{
    %         EX for predicted SQL with the input, which includes the user question and different numbers of retrieved tables on SpiderUnion and BirdUnion with SGPT-125M and SGPT-5.8B as the embedding.
    %         The best results with different models are annotated in \textbf{bold}.
    %         The results of $100$ retrieved tables on BirdUnion are not obtained because the input exceeds the model context length limit.
    %         % text-to-SQL实验结果：使用SGPT-125M和SGPT-5.8B，在SpiderUnion和BirdUnion+数据集上与DPR基线方法相比，执行准确率（EX）的结果。ours指本文的方法，表首行的数字代表输入的检索得到的表格的数量。-表示因输入超出模型上下文长度限制而未得到结果。
    %     }
    %     \label{tab:text-to-sq}
    % \end{table*}

\begin{table*}[htbp]
    \centering
    \small
    \begin{tabular}{ll|cccc|cccc}
        \toprule
        & & \multicolumn{4}{c|}{\textbf{SpiderUnion}} & \multicolumn{4}{c}{\textbf{BirdUnion}} \\
        \textbf{Model} & \textbf{Method} & \bm{$r@3$} &  \bm{$r@5$} & \bm{$r@10$} & \bm{$r@20$} & \bm{$r@3$} &  \bm{$r@5$} & \bm{$r@10$} & \bm{$r@20$}\\
        \midrule
        \multirow{3}{*}{SGPT-125M} & Single-hop & $43.9$ & $50.0$ & $53.2$ & $54.1$ & $11.2$ & $13.4$ & $17.1$ & $18.5$ \\
        ~ & CRUSH & $47.3$ & $50.9$ & \bm{$55.9$} & \bm{$59.6$} & $14.5$ & \bm{$17.1$} & $19.0$ & \bm{$20.5$} \\
        ~ & \ourmethod & \bm{$50.3$} & \bm{$54.1$} & $54.7$ & $57.4$ & \bm{$16.0$} & $16.8$ & \bm{$19.4$} & $20.0$ \\
        \cmidrule{1-10}
        \multirow{3}{*}{SGPT-5.8B} & Single-hop & $54.9$ & $60.6$ & $61.6$ & $63.7$ & $16.9$ & $17.3$ & $18.3$ & $20.4$ \\
        ~ & CRUSH & $49.8$ & $56.4$ & $60.3$ & $60.8$ & $16.8$ & $18.0$ & $19.7$ & $21.1$ \\
        ~ & \ourmethod & \bm{$62.5$} & \bm{$64.4$} & \bm{$64.4$} & \bm{$66.7$} & \bm{$20.9$} & \bm{$21.8$} & \bm{$22.0$} & \bm{$22.4$} \\
        \bottomrule
    \end{tabular}
    \caption{
        EX for predicted SQL based on the input, including the user question and varying numbers of retrieved tables on SpiderUnion and BirdUnion using SGPT-125M and SGPT-5.8B embeddings, compared with Sigle-hop and CRUSH.
        The best results with different models are annotated in \textbf{bold}.
    }
    \label{tab:text-to-sql}
\end{table*}



\subsection{Main Result} 
    The main results of our experiments are presented in Table~\ref{tab:main result}. 
    Compared to CRUSH, \ourmethod demonstrates significant improvements across various datasets and models of different scales, with an average enhancement of $5.7\%$ in recall and complete recall compared to the previous SOTA, which validates the effectiveness of our method. 
    From the table, we can also see that:

    \paragraph{The improvement of \ourmethod on BirdUnion is more significant than on SpiderUnion.}
        % 相比较在SpiderUnion数据集上的结果，我们的方法在BirdUnion+上的性能提升更加显著，因为BirdUnion+中的问题需要的表格更多，更需要多跳检索来提升检索性能。
        Since the questions in BirdUnion typically require more tables (see Table~\ref{tab:dataset}), requiring multi-hop retrieval of \ourmethod more to obtain multiple relevant tables, thereby enhancing retrieval performance.
        
    % \paragraph{\ourmethod improves the performance more with SGPT-125M compared with SGPT-5.8B.}
    %     % 我们的方法相比较使用SGPT-5.8B，使用SGPT-125M做编码器性能提升得更多, 因为SGPT-5.8B作为一个有更大参数规模的编码器，本身有更强的能力将问题和相关表格编码为相近的向量
    %     SGPT-5.8B, as an embedding with a larger parameter scale, has a stronger capability to embed questions and relevant tables into similar vectors, so the Rewrite benefits SGPT-5.8B less than SGPT-125M.
    %     The performance of CRUSH with SGPT-5.8B on both datasets is behind the baseline also because of the strong embedding capabilities of SGPT-5.8B.
    
    \paragraph{As the number of top-ranked tables grows, the retrieval performance of \ourmethod slows down.}
        % 我们的方法在top数较小的recall和complete recall上的提升更加显著，相比较在top数较大上的性能。
        % 因为提升top数字较大的指标需要检索到和用户问题极其不相似的表格，而我们的方法对于这样的问题提升性能更困难。
        Improving metrics with a high number of top-ranked tables necessitates retrieving relevant tables that are highly dissimilar to the user question, making the metrics challenging to enhance.
        % 尤其在一些指标上，我们方法的性能不如单跳和CRUSH，因为我们的方法在每一跳移除已经检索到的信息，导致检索更加专注于检索和用户问题很不相似的表格
        Especially, for some metrics (e.g., $k=20$, $r@20$), the performance of \ourmethod declines slightly because removing retrieved table information at each hop leads to a greater focus on retrieving tables that are highly dissimilar to the user question.

    % 
    \paragraph{Text-to-SQL Experiments}
        We conduct text-to-SQL experiments on the SpiderUnion and BirdUnion datasets using the user question and retrieved tables as the input, as shown in Table~\ref{tab:text-to-sql}. 
        % 我们的方法在text-to-SQL上的性能也打败了基线，展现出了和检索性能几乎一致的趋势，进一步证明了我们检索方法的有效性
        The performance of \ourmethod in text-to-SQL surpasses both Single-hop and CRUSH, exhibiting a trend similar to the retrieval performance, thereby further validating the effectiveness of our retrieval method. 
        % 随着输入表格变多，EX提升变缓，甚至有下降的趋势，因为过多不相关的表格令方法难以集中注意力于相关表格
        As the number of input tables increases, the EX improvement decelerates beyond the top $10$ tables due to the presence of too many irrelevant tables, which hinders the model from focusing on the relevant ones. 
        % 这也证明了在开放域text-to-SQL设置下提升较小top数的检索性能的必要性，因为虽然随着top数的增加，更有可能检索到更多多相关表格，但更多的表格输入不仅花销更大，而且不一定会带来text-to-SQL性能的上升 
        This also underscores the necessity of \ourmethod in enhancing retrieval performance on a small number of top-ranked tables in the open-domain text-to-SQL task.
    
\subsection{Ablation Studies}
\label{subsec:ablation}
    \begin{table*}[htpb]
        \centering
        \small
        \begin{tabular}{l|ccc|ccc}
            \toprule
            \textbf{Method} & \bm{$k=3$} &  \bm{$k=5$} &  \bm{$k=10$}  & \bm{$r@3$} & \bm{$r@5$} & \bm{$r@10$} \\
            \midrule
            \ourmethod & \bm{$65.0$} & \bm{$74.2$} & \bm{$81.0$} & \bm{$70.2$} & \bm{$77.5$} & \bm{$82.3$}\\
            \textit{w/o rewrite} & $46.2$ ($-18.8$) & $56.7$ ($-17.5$) & $67.2$ ($-13.8$) & $50.6$ ($-19.6$) & $60.7$ ($-16.8$) & $70.0$ ($-11.6$) \\
            \textit{w/o tabulation} & $54.6$ ($-10.4$) & $64.9$ ($-9.3$) & $75.5$ ($-5.5$) & $63.4$ ($-6.8$) & $72.5$ ($-5.0$) & $80.9$ ($-1.4$) \\
            \textit{w/o early stop} & $52.6$ ($-12.4$) & $64.9$ ($-9.3$) & $71.0$ ($-10.0$) & $57.1$ ($-13.1$) & $67.0$ ($-10.5$) & $72.2$ ($-10.1$) \\
            \bottomrule
        \end{tabular}
        \caption{
            The ablation results on evaluating \ourmethod, compared with splicing the question and previously retrieved tables (denoted as \textit{w/o rewrite}), rewriting to natural language question (denoted as \textit{w/o tabulation}), and without employing the mechanism of early stop (denoted as \textit{w/o early stop}) on SpiderUnion with SGPT-125M. 
            $k$ refers to the complete recall, and $r$ refers to the recall.
            The best results are annotated in \textbf{bold}.
        }
        \label{tab:ablation}
    \end{table*}
    % 为了证明重写为schema的必要性和有效性，我们对其进行了消融实验。
    To demonstrate the effectiveness of our method, we conduct ablation experiments on SpiderUnion, with results presented in Table~\ref{tab:ablation}.
    % 由于Spider是text-to-SQL的主流数据集
    We select SpiderUnion corresponding to Spider to perform subsequent experiments because Spider is the mainstream dataset for the text-to-SQL task.
    % SGPT-125M与SGPT-5.8B在不同setting下展现出同样的趋势，因此我们选取SpiderUnion with SGPT-125M进行消融实验
    Since SGPT-125M and SGPT-5.8B exhibit similar trends across different datasets and methods (as shown in Tables~\ref{tab:main result} and \ref{tab:text-to-sql}), we select SGPT-125M as the embedding model employed in the subsequent experiments to balance the embedding speed and the retrieval recall \cite{muennighoff-etal-2023-mteb_Text_Embedding_Benchmark}.

    \paragraph{The Effectiveness of Rewrite}
        % 为了证明在我们的方法中用LLM重写的有效性，我们对比了不重写直接将用户问题和每一跳的检索结果拼接的性能，是开放域QA中的常用方法
        To demonstrate the effectiveness of Rewrite which removes the retrieved table information from the user question, we compare its performance against the standard multi-hop retrieval method in open-domain QA, which is directly splicing the user question with retrieved tables at each hop without rewriting. 
        % 单纯拼接的方法性能显著且一致地下降，证明了我们方法中用LLM重写的有效性，也证明了通过移除已经检索到的信息来缓解相似不相关实体的必要性
        Compared with \ourmethod, the performance of splicing methods drops significantly and consistently, underscoring the effectiveness of Rewrite which alleviates retrieved tables similar to previously retrieved tables but irrelevant to the user question.


    \paragraph{The Effectiveness of Tabulation}
        % 为了证明我们的方法将问题改写为schema的有效性，我们将每一跳的问题改写为询问未检索到的信息的自然语言问题进行消融实验
        % 简写为tabulation
        To prove the effectiveness of transforming questions into a tabular format (abbreviated as tabulation), we rewrite the questions at each hop into natural language questions targeting to query unretrieved information.
        % 可以发现,相比改写为自然语言,我们的方法改写为schema显著提升了性能,证明了改写为schema的有效性
        The results indicate that, compared to rewriting to natural language, rewriting to tabulated questions significantly enhances performance, validating the effectiveness of tabulation in \ourmethod. 
        The prompt without tabulation is presented in Appendix~\ref{appendix:prompts for rewrite}. 

    \paragraph{The Effectiveness of Early Stop}
        % 为了证明我们方法中早停的有效性,我们对比了不早停,which不要求模型生成早停标记的结果
        To verify the effectiveness of early stop in \ourmethod, we compare the results without using this mechanism, where the model does not generate the special early stop mark.
        % 可以发现,没有早停的性能下降显著,证明在我们方法中引入早停机制有效地保证了性能
        The performance without the early stop is significantly degraded, which proves that incorporating the early stop mechanism in \ourmethod effectively guarantees the performance.
        
\subsection{Analysis}
    % 在分析实验中，我们主要采用complete recall $k=5$这一指标，并且在附录中解释了采用这一指标的原因
    In the analysis experiments, we study how different parameters affect the \ourmethod performance.
    We use $k=5$ as the evaluation metric, with detailed explanations provided in Appendix~\ref{appendix:the evaluation metric used in analysis experiments}. 
    % 我们在附录J中探讨了我们的方法的效率问题
    % 我们还探讨了SQL难度对我们方法的性能的影响，见附录~\ref{appendix:model details}
    Additionally, we discuss the the efficiency of \ourmethod in Appendix~\ref{appendix:discussion on efficiency} and the impact of SQL hardness on the performance in Appendix~\ref{appendix:impact of sql hardness}.

    % 为什么我们的方法相比较单跳方法有提升
    \subsection{Why \ourmethod improve compared with Single-hop method?}
        \begin{figure}
            \centering
            \input{fig/pieimprovement}
            \caption{
                The proportion of performance improvements due to solving different limitations by \ourmethod compared with Single-hop.
                % The number in parentheses in the legend represents the number of examples whose performance was improved due to solving this type of limitation.
                The number in parentheses in the legend represents the number of examples with the corresponding limitation type.
            }
            \label{fig:improvement}
        \end{figure}
        % 由于解决不同的限制而得到性能提升的比例
        % 图例中括号中的数字代表由于解决该类限制而得到性能提升的example的数量
        % 错误类型
        % 我们统计了我们方法因为解决这两个问题而提升性能的比例
        To explore why \ourmethod enhances retrieval performance, we analyze its improvement compared with Single-hop in Figure~\ref{fig:improvement}.
        % 我们的方法解决了这两种问题，并成功带来了性能提升
        The result indicates that the primary advantage of \ourmethod lies in its ability to mitigate the limitations of Similar Candidate and Semantic Gap. 
        (\emph{i})~Similar Candidate means that many candidate tables are similar to the question, complicating the retrieval of relevant tables. 
        \ourmethod alleviates the limitation by removing the retrieved information, allowing the model to focus on tables not yet retrieved. 
        (\emph{ii})~Semantic Gap refers to the semantic distinction between the natural language question and the relevant tables.
        % , which makes it difficult for the model to retrieve relevant tables. 
        \ourmethod organizes the user question into a table form and rewrites the question concerning the retrieved tables, aligning the question more closely with relevant tables in terms of domain and vocabulary, thus narrowing the semantic gap \cite{kothyari-etal-2023-crush4sql,knowledge-injection,li2024enhancingllmfactualaccuracy}. 
        Detailed examples illustrating the advantages of \ourmethod over Single-hop are provided in Appendix~\ref{appendix:detailed case study}, and the statistical criteria are discussed in Appendix~\ref{appendix:statistical criteria of limitations}
        % 我们统计的标准以及具体细节在附录中展现
        % The statistical criteria are presented in Appendix~\ref{appendix:statistical criteria of limitations}.


    % beam size对我们方法性能怎样影响
    % \subsubsection{Beam Size}
    \subsubsection{How Does Beam Size Affect the Performance?}
    \label{subsubsec:beam size}
         \begin{figure}
            \centering
            \input{fig/beam}
            \caption{
                The complete recall with different beam sizes on SpiderUnion with SGPT-125M.
            }
            \vspace{-1em}
            \label{fig:beam}
        \end{figure}
        
        % 为了观察不同的beam size对性能的影响，尤其是我们的方法采用beam search方法的有效性，我们对比了我们的方法在SpiderUnion数据集上用SGPT-125M做编码器在不同beam size设置下的性能，如表所示
        To observe the impact of different beam sizes on the retrieval performance, we compare the performance of our method using SGPT-125M as the embedding on the SpiderUnion dataset under the setting of different beam sizes, as shown in Figure~\ref{fig:beam}.
        % 当我们的方法不采用beam search的时候，即beam size为1的情况，我们的方法的性能下降的非常迅速，侧面证明了我们的方法可以通过beam search减轻错误级联的挑战、
        When our method does not employ beam search, i.e., with a beam size of $1$, performance degrades rapidly, indicating that beam search mitigates the effects of error cascade.
        % 并且，随着beam size的上升，complete recall整体呈明显的上升趋势直至beam size为5，之后的性能上升变平缓甚至下降，证明了在一定范围内，beam size的增大对性能的提升有促进作用，但过大的beam size引入了过多不相关表格，对性能的提升不再有帮助
        As the beam size increases, the complete recall shows a significant upward trend until reaching a beam size of $5$, beyond which performance either improves slightly or declines. 
        This indicates that while employing beam search enhances the performance of our method, a beam size greater than $5$ introduces too many irrelevant tables, resulting in higher computational costs without further performance gains.

    % 跳步数如何影响我们方法的性能
    % \subsubsection{Max Hop}
    \subsubsection{How Does the Number of Hops Affect the Performance?}
        \begin{table}[t]
            \centering
            \small
            \begin{tabular}{c|ccccc}
                \toprule
                \multirow{2}{*}{\textbf{Max Hop}} & \multicolumn{5}{|c}{\textbf{\#table}}\\
                 & \bm{$1$} & \bm{$2$} & \bm{$3$} & \bm{$\geq 4$} & \textbf{All} \\
                \midrule
                $1$ & $73.7$ & $59.8$ & $25.6$ & \bm{$50.0$} & $66.0$\\
                $2$ & $73.2$ & $77.6$ & \bm{$58.1$} & \bm{$50.0$} & $73.4$\\
                $3$ & \bm{$74.2$} & \bm{$78.0$} & \bm{$58.1$} & \bm{$50.0$} & \bm{$74.2$}\\
                $4$ & \bm{$74.2$} & \bm{$78.0$} & \bm{$58.1$} & \bm{$50.0$} & \bm{$74.2$}\\
                \bottomrule
            \end{tabular}
            \caption{
                Complete recall $k=5$ of \ourmethod with varying maximum hops. 
                We categorize the SpiderUnion dataset based on the number of relevant tables (denoted as \textbf{\#table}) per question. 
                \textbf{All} represents the undivided SpiderUnion dataset.
                The best results with different tables are annotated in \textbf{bold}.
            } 
            \label{tab:hop}
        \end{table}
        % 为了证明我们的方法多跳的有效性，我们对比了不同的最大跳步数的设置下的检索性能，如图所示
        To verify the effectiveness of multi-hop in our method, we conduct experiments on the SpiderUnion dataset, divided based on the number of relevant tables, using SGPT-125M as the embedding. 
        We compare the complete recall $k=5$ with varying numbers of maximum hops, as shown in Table~\ref{tab:hop}.
        The results indicate the following:
        % 我们的方法整体趋势为在跳步数大于等于所需表格数量时达到最佳性能
        (\emph{i})~The overall trend indicates that \ourmethod achieves the best performance when the number of maximum hops is greater than or equal to the required number of tables.
        % 所需表格为1个和2个的问题，均在3跳时达到最佳性能，因为我们的方法对于在前面跳步检索错误的问题能够提升性能，通过在每一跳移除已经检索到的信息，引导模型在后续跳步中检索没有被检索到的相关表格，
        (\emph{ii})~For questions requiring $1$ or $2$ tables, the best performance is achieved at a maximum hop of $3$. 
        Since \ourmethod can improve the performance of the questions that retrieve irrelevant tables in previous hops by removing the retrieved information, guiding the model to obtain unretrieved relevant tables in subsequent hops.
        % 其中，所需表格为1的问题在第2跳时略有下降，因为我们的改写是针对未检索到的表格，对于所需表格为1的问题改写可能会引入误差，不过这种误差在第3跳被消除
        (\emph{iii})~The performance for questions requiring a $1$ table slightly decreases with $2$ hops because removing retrieved information from such questions could easily introduce errors. However, this error is mitigated and eliminated at a maximum hop of $3$.
        % % 由于我们的方法有着严格的早停机制，所以所需表格为3个的问题在第3、4跳能够保持性能
        % 并且Complete recall $k=5$要求top 5个表格中包含全部正确表格，对于需要4个表格的问题较难提升，所以它们的性能在多跳中保持不变
        (\emph{iv})~The performance of requiring $\geq 4$ tables remains unchanged across multiple hops because improving complete recall $k=5$ necessitates that the top $5$ retrieved tables include all relevant tables, which is challenging.

    % \subsubsection{Average Rank}
    \subsubsection{Can \ourmethod Reduce the Average Rank of Relevant Tables?}
        \begin{figure}[t]
            \centering
            \begin{subfigure}[b]{0.48\linewidth}
                \centering
                \input{fig/rank}
                % \caption{The average rank of relevant tables with different numbers of max hop on the SpiderUnion using SGPT-125M with \ourmethod.}
                % \label{fig:rank}
            \end{subfigure}
            \hfill % 在两个子图之间添加一些水平空间
            \begin{subfigure}[b]{0.48\linewidth}
                \centering
                \input{fig/stop}
                % \caption{The proportion that still retrieves at each hop when the max hop is $3$ on the SpiderUnion using SGPT-125M with \ourmethod.}
                % \label{fig:stop}
            \end{subfigure}
            \vspace{-1em}
            \caption{
                The left part is the average rank of relevant tables with different numbers of max hops on the SpiderUnion with \ourmethod.
                The right part is the proportion of questions that are not early stopped with different hops on the SpiderUnion with \ourmethod.
            } % 如果需要，可以取消注释这一行以添加总标题
            \label{fig:rank}
            \vspace{-1em}
        \end{figure}
        % 为了验证我们的方法可以提高相关表格的平均排名，我们统计了不同最大跳步数时相关表格的平均排名，如图所示
        To verify the effectiveness of \ourmethod in improving the average rank of relevant tables, we calculate the average rank at different maximum hops, as shown on the left part of Figure~\ref{fig:rank}. 
        From the figure, we can see that \ourmethod significantly enhances the average rank of relevant tables, with the most notable improvement occurring at a maximum hop of $2$. 
        This is because most questions in SpiderUnion require $1$ or $2$ tables (see Table~\ref{tab:dataset}), requiring two hops to obtain unretrieved relevant tables.
        Conversely, the improvement at a maximum hop of $3$ is weak, not only because of the limited number of questions requiring $\geq 3$ tables but also due to the early stop mechanism, which causes most questions to cease retrieval before the third hop.

        % 我们方法执行的不同跳步数的比例，与表中不同跳步数对应的表所占的比例基本一致
        As illustrated in the right part of Figure~\ref{fig:rank}, the proportion of different hops performed by our method is almost the same as the proportion of the table corresponding to the different table numbers in Table~\ref{tab:dataset}.
        % 大部分的用户在第三步的时候已经停止检索，因此我们设置最大跳步数为3是合理的
        Besides, most user questions have stopped retrieving in the third hop, so it is reasonable to set the maximum hop steps to $3$.

    % 我们的方法错误级联问题严重吗
    % \subsubsection{Error Cascading}
    \subsubsection{How Does the Previous Errors Affect Subsequent Performance?}
        To examine the error cascades in \ourmethod, we analyze the number of errors with different recalls that occurred in different hops.
        We compare the performance of $r@5$ during multiple hops, categorizing the questions into $r@5=0$, $0<r@5<1$, and $r@5=1$ based on the results in the first hop, as illustrated in Figure~\ref{fig:error}. 
        We use SGPT-125M as the embedding model and conduct experiments on the SpiderUnion dataset, with a beam size of $5$ and a maximum hop of $3$.
        \begin{figure}
            \centering
            \input{fig/error}
            \caption{
                % 第一跳不同区间的召回率对应的example在后续跳步的召回率，证明我们的方法错误级联现象并不严重
                The $r@5$ during multiple hops, categorizing according to the $r@5$ in the first hop which falls into different intervals, demonstrates that the cascading effect of our method is not significant.
            }
            \label{fig:error}
        \end{figure}
        
        % 可以发现，我们的方法的错误级联现象并不严重，并且显著被多跳检索带来的性能提升弥补。
        The error cascades in \ourmethod is minimal and is significantly compensated by the performance improvements brought about by multi-hop retrieval. 
        We analyze these three categories of questions separately.
        % 对于在第一跳检索的结果的recall@5=0的问题，也就是说，第一跳保留的5个表格中全部为不相关的表格，把检索到的信息从用户问题中移除，可以一定程度上排除之前跳步检索到的不相关表格的干扰
        (\emph{i})~For questions whose $r@5 = 0$ in hop $1$, the top $5$ tables retrieved are all irrelevant. 
        \ourmethod improves performance because removing the retrieved information from the user question can eliminate the interference of irrelevant tables retrieved in the previous hops.
        % 对于在第一跳检索的结果的0 < recall@5 < 1的问题，我们的方法可以在第2跳显著提升性能，也就是说，即使第一跳保留的top 5个表格中有不相关的表格，我们的方法也可以在后续跳步中通过移除已经检索到的信息专注检索未被检索到的表格，以此提升性能。我们的方法在第3跳的性能略有下降，主要因为SpiderUnion中超多90%的问题只有少于等于2个相关表格，多余的跳步会引入误差
        (\emph{ii})~For questions with $0<r@5<1$ in hop $1$, there are irrelevant tables among the $5$ retained tables. 
        Our method significantly enhances performance in hop $2$ by extracting the retrieved table information from the user question and focusing on retrieving unretrieved relevant tables. 
        Performance in hop $3$ is slightly reduced, mainly because most questions in SpiderUnion have $\leq 2$ relevant tables (see Table~\ref{tab:dataset}), and additional hops may introduce errors. 
        % 对于在第一跳检索的结果的recall@5=1的问题，我们的方法在第2跳和第3跳的性能略有下降，因为如果第一跳就检索到全部相关的表格，我们的方法后续的跳步可能会引入少量误差。
        (\emph{iii})~For questions whose $r@5 = 1$ in hop $1$, performance in hops $2$ and $3$ is slightly reduced as all relevant tables are retrieved, causing subsequent hops to introduce a small amount of error.
        
    
    \subsection{Case Study}
        \begin{figure}
            \centering
            \includegraphics[width=1\linewidth]{fig/case.pdf}
            \caption{
                A case study comparing \ourmethod with CRUSH. 
                \introgreen{Green} indicates relevant tables, while \introred{red} indicates irrelevant ones. 
                Each table is represented as “database name.table name(column names)”.
                $r$ denotes recall.
            }
            \label{fig:case}
        % 每个表格被表示成“”的形式
        \end{figure}
        % 举一个例子说明用Baseline做不对，用我们的方法能做对
        We demonstrate a case study with \ourmethod compared with CRUSH, as shown in Figure~\ref{fig:case}.
        % 因为受限于单跳检索，表格2的检索依赖于表格1
        We can see that CRUSH fails to retrieve the table \textit{"world\_1.countrylanguage"} within the top $3$ results due to its single-hop retrieval limitation, as the retrieval of table \textit{"world\_1.countrylanguage"} relies on the table \textit{"world\_1.city"}.
        % 相反，我们的方法采用了多跳检索，并设置beam size为3，增加了在每一跳选择相关表格的概率
        In contrast, \ourmethod employs multi-hop retrieval with a beam size of $3$, increasing the probability of selecting relevant tables at each hop. 
        % 并且，在每跳移除已经检索到的信息，帮助模型检索到没在第一跳被检索到的\textit{"world\_1.countrylanguage"}
        Additionally, we eliminate the retrieved information in \textit{"world\_1.city"} from the question, which aids the model in retrieving \textit{"world\_1.countrylanguage"} that was previously missed. A detailed comparison with additional methods is provided in Appendix \ref{appendix:detailed case study}.

